The Geometry of Deep Networks: Power Diagram Subdivision

We study the geometry of deep (neural) networks (DNs) with piecewise affine and convex nonlinearities. The layers of such DNs have been shown to be {\em max-affine spline operators} (MASOs) that partition their input space and apply a region-dependent affine mapping to their input to produce their output. We demonstrate that each MASO layer's input space partitioning corresponds to a {\em power diagram} (an extension of the classical Voronoi tiling) with a number of regions that grows exponentially with respect to the number of units (neurons). We further show that a composition of MASO layers (e.g., the entire DN) produces a progressively subdivided power diagram and provide its analytical form. The subdivision process constrains the affine maps on the (exponentially many) power diagram regions to greatly reduce their complexity. For classification problems, we obtain a formula for a MASO DN's decision boundary in the input space plus a measure of its curvature that depends on the DN's nonlinearities, weights, and architecture. Numerous numerical experiments support and extend our theoretical results.

==> biasless.tex <==
\iffalse
\section{Region Margins}
\label{sec:margin}

We developed in the last two sections the input space partitioning of DN units and layers. We now propose to actively leverage those findings by deriving a margin measure of given samples. That is, \textit{how close is a given point from its closest region boundary}. We first derive how this can be computed simply and how can this be used for qualitative analysis of DNs. We then extend this finding by providing an additional penalty term that can be used in addition of standard loss function and maximizing the margin between each points and their closest region boundary.






\subsection{Minimum Region Margin}
Given a layer power diagram in general, we aim at providing a measure of how close is a given point $\bx$ to its closest region boundary. In general, it is not computationally tractable to discover all the boundaries of a region and enforcing that the closest boundary is at a specific distance is enough to ensure that $\bx$ lies far away from all the boundaries of its region. 
Second, based on Sec.~\ref{sec:layer}, we know the analytical form of the layer power diagram. 
Let first remind the following distance between a query point $\bx$ and an hyperplane with parameters $\alpha$ and $\beta$ which is given by $ \frac{| \langle \alpha,\bx \rangle +\beta |}{\| \alpha \|_2}$.
We can now provide the following result where we focus on layers with $R=2$ nonlinearities.
\begin{thm}
The distance between a point $\bz^{(\ell-1)}$ and its nearest layer region boundary is given by
\begin{align}
    m^*(\bz^{(\ell-1)},l,k)=\min_{k} \frac{| \langle [A^{(\ell)}]_{k,2,\bigcdot},\bz^{(\ell-1)} \rangle +[B^{(\ell)}]_{k,2} |}{\| [A^{(\ell)}]_{k,2,\bigcdot}\|_2} 
\end{align}
\end{thm}
First, we can leverage this measure to define a ball around a given point in which any input will be associate to the same region. Given an input $\bz^{(\ell-1)}$, we define its linear ball $\epsilon$ as $\mathcal{B}(\bz^{(\ell-1)};m^*(\bz^{(\ell-1)},l,k)$.
\begin{cor}
Any input belonging to $\mathcal{B}(\bz^{(\ell-1)};m^*(\bz^{(\ell-1)},l,k)$ are in the same region as $bz^{(\ell-1)}$.
\end{cor}
\subsection{Application: Layer Region Measures}
We experiment by training different models and showing for each layer the linear ball of different dataset.
\subsection{Application: Margin Maximization}

This type of weight constraint translates in general in the deep learning community into the use of specific topologies s.t. convolutional, fully-connected, maxout and so on. 
In general, an important duality is made between a fully-connected and a convolutional layer. The latter allows to constrains the layer input space partitioning by having weights localized in the spatial dimension. That is, at a specific output unit position, the input space region has boundaries parallel to the axis on all the dimensions far away from this output spatial position. For images, such topologies are often taken by default due to images being characterize by localized features that are in general independent from each other if spatially spaced.
While this intuition holds, we now propose some experiments to highlight some new findings. 
We experiment by taking $3$ topologies (varying number of units) for DN made of a first block of $3$ layer being either convolutional or fully-connected then in both cases followed by $2$ fully-connected ones. To have exact comparison in term of partitioning, the fully-connected layers have output units set to be the same as the number of output units of convolutional layers (that is, number of filters times number of spatial positions). See Appendix~\ref{app:topology_description} for details on the training procedure and all details and architectures.
We propose results in Table.~\ref{tab:cnn_vs_mlp}
\begin{table}[t]
\small
    \centering\setlength\tabcolsep{1.3pt}
\begin{tabular}{|l|c|c|c|c|}\hline
Model & Fashion & SVHN & CIFAR10 & CIFAR100 \\ \hline \hline
allCNN1 &\textbf{90.5} $\pm$ 0.2 & 85.4 $\pm$ 0.4 & \textbf{56.9} $\pm$ 0.2 & \textbf{27.8} $\pm$ 0.3 \\\hline
allDENSE1 &89.9 $\pm$ 0.2 & \textbf{87.7} $\pm$ 0.2 & 53.1 $\pm$ 0.7 & 15.0 $\pm$ 0.5 \\\hline \hline
allCNN2 &90.6 $\pm$ 0.2 & 85.0 $\pm$ 0.3 & 57.2 $\pm$ 0.4 & \textbf{27.6} $\pm$ 0.2 \\\hline
allDENSE2& \textbf{90.8} $\pm$ 0.2 & \textbf{88.1} $\pm$ 1.6 & \textbf{58.4} $\pm$ 0.7 & 18.3 $\pm$ 0.4 \\\hline \hline 
allCNN3 &90.4 $\pm$ 0.2 & 85.4 $\pm$ 0.1 & 57.1 $\pm$ 0.5 & \textbf{27.8} $\pm$ 0.2 \\\hline
allDENSE3 &\textbf{91.4} $\pm$ 0.3 & \textbf{89.8} $\pm$ 0.2 & \textbf{62.5} $\pm$ 0.6 & 21.0 $\pm$ 0.4 \\
\hline
\end{tabular}
    \caption{Average (over 10 runs) test set accuracy for the various DNs comparing fully-connected models with convolutional models in which $L$ and $D^{(\ell)},\forall \ell$ are equal. As can be seen the test set accuracy is very similar in most cases. As $D^{(\ell)}$ increases as the DENSE topology outperforms the CNN one. See Appendix~\ref{app:topology_description} for details.}
    \label{tab:cnn_vs_mlp}
    \normalsize
\end{table}
Due to this the fully-connected has much more degrees of freedom and being unconstrained, can represent a much broader class of functions. In term of input space partitioning, the DENSE topologies are unconstrained whereas the CNN ones have regions parallel to most of the input space axis due to their high localization of their filters. 
As a result, \textit{constraining the shape of the regions imposes a structural bias controlling the train/test set accuracy gap.}
\fi

\iffalse

\section{Interpretable Deep Networks via Biasless Layers}


%PCAnet \cite{chan2015pcanet} binary hashing and histogram statistics as well as hand-crafted architectures.


We developed in the last section various results relating DN layers and input space partitioning via power diagrams, a generalization of Voronoi Diagrams. While this led to various experiments to better characterize and understand the layer input space partitioning, we now propose to study particularly the biasless case (or zero bias). We demonstrated in Table~\ref{tab:VQ_bias} that such cases do not impact performances, yet, we now see that it greatly simplifies interpretability and visualization of the power diagram. We first demonstrate that in this case, the layer input space corresponds to a Voronoi Diagram. 






Even though the actual number of regions grows exponentially w.r.t. the number of units, in practice, most of those regions might live in a part of the input space which is never reached by a given dataset. 
For example, we depict some centroids of the layer that in practice shall never be reached unless by abnormal inputs.
\iffalse
\subsection{Initialization and Batch-Normalization}
At initialization, the sphere is randomly covered. batch-normalization, when applied onto the input of the layer allows to spread the input data roughly around the origin and thus maximizes the number of non empty regions and diversify the active regions.
\randall{plotof what batch norm does, it centers data and scales them then you apply the sphere clustering, also different nonlninearities, which nonlinearity ? the one spanning good the dataset spread}
\subsection{Application: New Batch-Normalization, }
\subsection{Application: Unsupervised Layer Training}
We propose the following Lloyd inspired training procedure.
We explore different strategies: greedy, global. For those case we train in an unsupervied manner all the layers (but the last) and then once convergence has been reach, those layers are frozen and only the last layer is trained. This highlights the ability of the unsupervised training to characterize inputs. 
\subsection{Application: Clustering}
We do the same as above but also train in this manner the last layer and use this for clustering task and thus at not time training is done with the information of the labels.
\subsection{Recovery Result}
From the residual PCA paper with uniform sampling

\fi





\section{Maximum Inner Product Search}
\url{https://arxiv.org/pdf/1507.05910.pdf}

\fi

==> bounds.tex <==




\subsection{Bounds on the Number of cells in a Deep Network}

The above provides upper bound
In fact, the only way to reduce the number of cell from $R^K$ is to have low-rank weights and/or having same bias for multiple units. Note that this result assumes to consider the whole infinite input space.
Based on the above results, we obtain the following direct applications.
%
\begin{prop}
\label{prop:tuerie}
The number of cells in the layer input space partitioning ($R^K$) grows exponentially in the number of units $K$ (and thus parameters) of the layer.
\end{prop}
%


In this section, we provide bounds on the number of cells that the subdivision performed by the DN induces. Notice that here, we will assume that the nonlinearity is with $R=2$ throughout the model (as with ReLU, leaky-ReLU or absolute value).
We first provide some intuitions regarding how a subdivision is performed and how it can be theoretically counted. Denote by $H^{(\ell)}_k$ the number of broken segments created at layer $\ell$ for unit $k$: 
\roro{deja definie au dessus}
\begin{align}
    H^{(\ell)}_k=\sum_{\omega \in \Omega^{(1 \leftarrow \ell-1)}_{q^{(1)},\dots,q^{(\ell-1)}}} 1(\{Ax+b=0\}\cap \omega \not = \emptyset)
\end{align}
Hence, $H^{(\ell)}_k$ counts the number of cells in the current partitioning $\Omega^{(1 \leftarrow \ell-1)}_{q^{(1)},\dots,q^{(\ell-1)}}$ that unit $k$ of layer $\ell$ subdivides.
Since for each cell, the unit will either subdivide it into $2$ cells or leave it as is, we can thus have the exact number of newly introduced cell from the current layer $\ell$ as  
\begin{equation*}
    R^{(\ell)}= R^{(\ell-1)}+ \sum_{k=1}^{D(\ell)}H^{(\ell)}_{k},
\end{equation*}
where $R^{(\ell)}$ defines the number of cell at layer $\ell$, that is, $R^{(\ell)}={\rm Card}(\Omega^{(1 \leftarrow \ell-1)}_{q^{(1)},\dots,q^{(\ell-1)}})$ and $D(\ell)$ is the number of units at layer $\ell$. The number of cells at layer $\ell$ is the number of cells at layer $\ell-1$ plus the number of pieces of the piecewise affine hyperplane created by each unit of the layer $\ell$. With this characterization, we now provide an upper and lower bound on the number of cell of a DN with $L$ layers. In particular, we will focus in the rate of increase of $R^{(\ell)}$ with depth $\ell$.
\\
{\bf Upper Bound:}
Without any further assumption regarding the organization of the cells, one can derive the following upper-bound,
\begin{prop}
The number of cells at layer $\ell$ is upper bounded by
\begin{align}
    R^{(L)} \leq &R^{(1)} \left ( \prod_{\ell=1}^L(1+K^{(\ell)}) \right )
    \leq R^{(1)}\left(\sum_{b\in\{0,1\}^{L}}\prod_{\ell=1}^L(K^{(\ell)})^{[b]_l}\right)
    \leq R^{(1)}\left(\sum_{b\in\{0,1\}^{L} -\{1,\dots,1\}}\prod_{\ell=1}^L(K^{(\ell)})^{[b]_l}+\prod_{\ell=1}^LK^{(\ell)}\right)
\end{align}
\end{prop}
\begin{proof}
The proof is done by induction the layer $1$ gives
$R^{(1)}$ cells. Then,
\begin{equation*}
    R^{(2)} = R^{(1)} + K^{(2)}R^{(1)}=R^{(1)}(1+K^{(2)}),
\end{equation*}
wich can be translated as, each unit of layer $2$ splits the layer $1$ into two pieces (non-linearity is piecewise with two pieces). Thus the number of new cells created by this subdivision is equal to the number of units times the number of cells in the previous layer, i.e: $K^{(2)}R^{(1)}$. 
\end{proof}
\begin{cor}
The Maximum number of cells of a DN increases exponentially w.r.t. the depth.
\end{cor}
This result has been often characterized \cite{}.
\\
{\bf Lower Bound:}
In order to derive a lower bound, we first need to characterize a uniform partitioning in a broad sense.
\begin{defn}
A partitioning $\Omega$ of $\mathbb{R}^D$ is denoted as $D$-uniform if
\begin{align}
    {\rm Card}\{\partial \Omega \cap \{\sum_{k=1}^v w_k[\alpha]_k,\alpha \in \mathbb{R}^v\}\}=\kappa_d, \forall w_k \in \mathbb{R}^D, \forall v=1,\dots,D
\end{align}
\end{defn}
With this broad sense of uniform partitioning, we can now provide a lower bound on the number of DN cells. To do so, we assume that ${\rm Card}(\Omega^{(1 \leftarrow \ell-1)}_{q^{(1)},\dots,q^{(\ell-1)}})$ is $D$-uniform.
In that case, the minimum number of cells that unit $k$ of layer $\ell$ can subdivide is given by the number of cells present in the current partitioning along any directional slice. As we assume the partitioning is uniform, the direction of the slice does not impact the average number of cells crossed. Let first study how many cells of a $D$-dimensional uniform partitioning a slice of dimension $\kappa$ intersects.
\begin{lemma}
Uniform partitioning of $\mathbb{R}^D$ with $K$ cells. Intersection with linear manifold of dimension $P$, it crosses on average $(K)^{\frac{Q}{K}}$ cells.
\end{lemma}
With the above lemma, we are now able to provide the following lower bound.
\begin{prop}
Given a uniform division of the cells, at layer $\ell$ defined by $R^{(\ell)}$ is lower bounded by,
\begin{equation}
    R^{(\ell)} \geq R^{(\ell-1)} + K^{(\ell)} (R^{(\ell-1)})^{\frac{D-1}{D}}.
\end{equation}
\end{prop}
\begin{proof}
Let's denote by $D(\ell)$ the dimension of layer $\ell$. Given the uniform assumption, the number of cells at layer $1$ per dimension is given by $R^{(1)}^{\frac{1}{D^{(1}}}$. In fact, it is clear that with the uniform assumption, each dimension share the same number of cell being the $D(1)$-roots of the total number of cells. Now, an hyperplane splits this space will create a minimum of $((R^{(1)})^{\frac{1}{D(1)}})^{D(1)-1}$ cells. In fact, the initial number of cell is duplicated at minimum on $D(1)-1$ dimension which is the dimension of the hyperplane. Thus each unit of the $2$nd layer creates at least $(R^{(1)}^{\frac{1}{D(1)}})^{D^{(1)-1}}$, which is $K^{(2)}((R^{(1)})^{\frac{1}{D(1)}})^{D(1)-1}$ new cells.
\end{proof}
\begin{cor}
The number of cells in a DN increases superlinearly w.r.t. depth.
\end{cor}
\begin{proof}
The thing with arithmetic suite etc
\end{proof}
This result is crucial as it demonstrates that even in the worst case (of introducing the least number of splits) the number of cells will still increase at a super linearly rate w.r.t. the depth of the DN.

\tiny








\section{Code Maximization}
In order to easily visualize what types of inputs are present in each cell we perform a similar thing as the activity maximization. Yet the difference is that we do not maximize the output of a unit but rather want to get an image s.t. it has some pre-imposed VQ.
We demonstrate that  when imposing the whole VQ we get the same image. We then do variety of experiments with constraints on only some parts of the VQ and show how the cells change.
\subsection{Active cell Sampling}
We do now know a priori how to sample points belonging to a specific VQ code or cell
\begin{align}
    \text{ find $\bx$ s.t. } d(Q(\bx),Q^*)=0,
\end{align}
where $Q^*$ is a given VQ code and $d$ is a distance. In particular we use the Hamming distance with explicit layer as in
\begin{align}
    d^{\mathcal{L}}(Q_1,Q_2)=\sum_{\ell \in \mathcal{L}} d(Q_1^{(\ell)},Q_2^{(\ell)}).
\end{align}
In particular if we impose for example just the code for some layers s.a. the deeper ones. 

We initialize with random noise and samples form the training set.
\begin{align}
    \bx^*(Q^*,\mathcal{L})=\argmin_{\bx}d(Q(\bx),Q^*).
\end{align}
We can do this by using the Soft VQ which allows to backpropagate through a code and thus perform gradient descent to solve this minimization problem. This is an infinite set but we sample many and show them.

CONJECTURE:
\begin{itemize}
    \item Layer 1 only is about euclidean distance (DUH)
    \item Last layer is about labels
    \item ALL layers is super small cell just 1 image in
    \item this sample things that can be classified (using just the last layer VQ)
    \item Future work: use the code for better data modeling, not just output
\end{itemize}






\normalsize




\iffalse
\section{Active Subdivision Scheme}
\randall{still working on this one but will be great}

FORGET BELOW:
LATERAL CONNECTION WITH MULTIPLICATIVE WEIGHTS BETWEEN 0 AND 1 MULTIPLYING THE VQ STATES ! NO FROM THE VQ STATE TO THE OTHER UNIT OUTPUTS YES THIS IS A WIN
THIS ENABLES MULTISCALE THING AND IT IS FINISHED
DO A FULL MATRIX AND PLUG IT WITH FIXED DIAGONAL.
NEED TO BE A ONE HOT VERSION >< OF Q
MAYBE DO AVERAGE OF MULTIPLE GUYS GOING TO THE SAME ONE YES !
OR MAYBE THE MIN AFTER SIGMOID

2 networks but sharing the $Q$ ! an the other one has whatever weights it wants.
So it might not even be continuous lol. And then use it with a sigmoid gated. THEN IT MUST HAVE THE SAME cell !!!!!!! AND WILL DECIDE IF YOU KEEP SUBDIVIDING OR NOT. because the ones with 0 wont be dealt with with the next layer.BUT NEED TO FEED EVERYTHING INTO THE CLASSIFIER ! with 1-sigmoid.
MAYBE NOT SHARE Q AND ALL JUST NEED TO FIND A WAY TO GET A MAPPING LEARNABLE FROM ONE HOT GUYS TO A 0 OR 1. MAYBE IT WORKS BUT NEEDS TO BE INTO A 1HOT FORMAT SO MULTIPLY ALL BYT 2 AT LEAST BUT IT IS ok ?


Product of classifiers, one for each layer (REVERSE RESI FROL $\ell$ to $L$ ! 
OROROR
MULTIPLICATIVE RESNET IT IS THE SAME (with RELU)

EXPERIMENT DIFFICULT FOR DN:
2D HALF CIRCLE WITH VERY NONLINEAR CIRCULAR PART AND THEN STRAIGHT LINES

\fi

==> kmean.tex <==
\section{Extension: Factorial K-Mean}


\begin{align}
    z=&A_{r^*}x+B_{r^*},\text{ s.t. }\;r^*=\argmin_r \|x-\mu_{r} \|+b_{r} &&(MASO)\\
    z=&A_{r^*}x+B_{r^*},\text{ s.t. }\;r^*=\argmin_r \|x-\mu_{r} \| &&(VMASO)
\end{align}

\begin{thm}
The DVL is a piecewise affine, continuous mapping for any parameters $A^{(\ell)}$, and is also convex if $A^{(\ell)}$ are orthogonal .
\end{thm}

\begin{thm}
The optimization problem can always be cast into a binary optimization problem for standard DN nonlinearities in which $R^{(\ell)}=2,\forall \ell$.
\end{thm}

image co-segmentation \cite{joulin2010discriminative}, community discovery \cite{chan2011convex,he2016joint}, graph matching \cite{zaslavskiy2009path} or Markov random Fields \cite{boykov2001fast}.


there are two types of methods: relaxation and equivalent. The first optimizes over a relaxed optimization problem and then 
Review, exact penalty method \cite{yuan2017exact}


We focus on linear programming relaxation in which we optimize a continuous vector and then round up the final solution \cite{komodakis2007approximate}. This method suffers some limitation especially if there exist numerous constraints on the form that the optimal binary vector should take. In our case, we have no constraints and thus rely on this method. We couple this approach with the one of \cite{candes2015phase}, in which a careful initialization is used prior to performing the relaxed optimization.

In our case we initialize with the forward pass of a DN by setting the vector as the soft probability \cite{smaso}.


Note that despite the need to optimize the region allocation, this model still benefits form exactly the same as Prop.\ref{prop:parameters} regarding the number of regions growing exponentially w.r.t. the number of parameters.







Exactly the same number of parameters as standard K-mean with $k=10$.



==> unit.tex <==
\section{Input Space Geometry of a Single Unit}
\label{sec:unit_section}

We study the input space partitioning of a single unit which is a max-affine spline.
We begin by introducing the notions of a Voronoi diagram and a power diagram (PD).
\medskip


\begin{defn}
A partitioning $\Omega=\{\omega_1,\dots,\omega_C\}$ made of $C$ disjoint regions s.t. $\cup_{\omega \in \Omega} =\mathcal{X}$ can be obtained via $\omega_r = \{ \bx \in \mathcal{X} :r(\bx)=r\}, r=1,\dots,C$ with
\begin{align}
    r(\bx)=&\argmin_k \|\bx - [\mu]_{k,\bigcdot} \|^2   \},&\text{ Voronoi Diagram (VD) \cite{aurenhammer1991voronoi}}\label{eq:region_vd}\\
    r(\bx)=&\argmin_k \|\bx - [\mu]_{k,\bigcdot} \|^2+[{\rm rad}]_k \},&\text{ Power Diagram (PD) \cite{aurenhammer1988geometric}}\label{eq:region_pd}
\end{align}
$\forall r$, where $[\mu]_{k,\bigcdot}$ is denoted as a centroid and $[{\rm rad}]_k$ is a radius, this is known as the {\em Laguerre distance}\cite{imai1985voronoi}.
\end{defn}

Clearly, the PD is a generalization of the VD by introduction of an external radius term.
In general, a PD is defined with 
$[{\rm rad}]_k^2$ to provide additional insights which require nonnegativity. However, the PD is the same under global shifting as $\argmin_k \|\bx - [\mu]_{k,\bigcdot} \|^2+[{\rm rad}]_k =\argmin_k \|\bx - [\mu]_{k,\bigcdot} \|^2+[{\rm rad}]_k +Q$. Thus, we allow for negative radius as they can always be shifted back to nonnegative by setting $Q=-\min_k [{\rm rad}]_k$.
For additional geometric insights on VDs and PDs, please see Appendix \ref{appendix:extra_geometric}. 
On a counterintuitive note, due to the latter radius $[{\rm rad}]_k$, the centroid $[\mu]_{k,\bigcdot}$ of a PD cell does not necessarily reside inside that cell.
We also denote directly the partitioning of a space $\mathcal{X}$ by a PD via 
\begin{align}
\Omega = \PD(\mathcal{X};\{([\mu]_{r,.},[{\rm rad}]_r),\forall r\})=\{\omega_1,\dots,\omega_C\}\text{ with $\omega_k$ given by (\ref{eq:region_pd})}.\label{eq:pd_def}
\end{align}
\randall{figure, VD versus PD}







\subsection{Geometrical Interpretation of the Unit Output Calculation}
\label{sec:geometric_unit}
Since we first focus on a single unit (aka ``neuron'') in a DN layer; we omit the $(\ell)$ superscript for brevity, and denote the layer input by $\bx \in \mathbb{R}^D$ and the unit output by $\bz_k(\bx) \in \mathbb{R}$ with $\bz_k$ a MAS (recall Section~\ref{sec:back}). Let
%
\begin{align}
\bz_k(\bx)=\max_r \Epsilon_{k,r}(\bx)=\max_r \left\langle [A]_{k,r,\bigcdot},\, \bx \right\rangle +[B]_{k,r},
\label{eq:E}
\end{align}
%
where $\Epsilon_{k,r}(\bx)$ is the projection of $\bx$ onto the hyperplane parameterized by the slope $[A]_{k,r,\bigcdot}$ and offset $[B]_{k,r}$.
Define the image of the unit conditioned on some subset $S\subset \mathcal{X}$, being the collection of outputs for any possible input $\bx$ belonging to $S$, as
%
\begin{equation}
{\rm Im}_{S}(\bz_k):=\bz_k(S) = \left\{ \max_{r} \Epsilon_{k,r}(\bx),\forall \bx \in S \right\},\label{eq:z_boundary}
\end{equation}
%
where ${\rm Im}_{\mathcal{X}}(\bz_k)$ recovers that standard image definition. Also, let $\Epsilon_{k,r}^{+}$ denote the half-space consisting of the set of points above the hyperplane $\Epsilon_{k,r}$ in $\mathcal{X}\times \mathbb{R}$ for each $r$
\begin{equation}
    \Epsilon_{k,r}^{+} = \{(\bx,y) \in \mathcal{X}\times \mathbb{R} : y \geq \Epsilon_{k,r}(\bx) \}.
\end{equation}
We characterize the geometry of the unit mapping as follows.




\begin{prop}
The unit output  $\bz_k(\mathcal{X})$ from (\ref{eq:z_boundary}) corresponds to the boundary of a convex polytope $\mathcal{P}$ as
\begin{equation}
    \bz(\mathcal{X}) = \partial \mathcal{P}_k \text{ where } \mathcal{P}_k = \cap_{r=1}^R \Epsilon_{k,r}^{+}.
    \label{eq:polytope}
\end{equation}
\label{prop:singleunit}
\end{prop}

As such the unit output $[\bz]_k$ corresponds to the projection of the input $\bx$ onto the boundary $\partial \mathcal{P}_k$ of the polytope $\P_k$.
\randall{figure do it ! to explain fomr W to A}










\subsection{Input Space Partitioning of a Single Unit} 

We now derive the input space partitioning of a unit $[\bz]_k$ with $k\in \{1,\dots,K\}$. Recall from Proposition~\ref{prop:singleunit} that a unit projects the input $\bx$ onto the polytope boundary $\partial \mathcal{P}_k$. In particular, it is mapped onto the polytope face, defined by $r(\bx)$, that maximizes the projection output
\begin{align}
    r(\bx) =& \argmin_{r=1,\dots,R} \left\| \bx - [\mu]_{k,r} \right\|^2 + [{\rm rad}]_{k,r} = \argmax_r \Epsilon_{k,r}(\bx)
\end{align}
 with 
$[\mu]_{k,r}=[A]_{k,r,\bigcdot}$, and 
$[{\rm rad}]_{k,r}=-2[B]_{k,r}-\|[A]_{k,r,\bigcdot}\|^2,\forall r\in \{1,\dots,R\},\forall k$.
%$
%r(\bx) = \argmax_{r=1,\dots,R}  \left\langle [A]_{k,r,\bigcdot}, \bx \right\rangle +[B]_{k,r}=\argmin_{r=1,\dots,R} \left\| \bx - [A]_{k,r,\bigcdot} \right\|^2 + [{\rm rad}]_{k,r} \:,
%$ with $[{\rm rad}]_{k,r}=-2[B]_{k,r}-\|[A]_{k,r,\bigcdot}\|^2$. The left hand side follows directly from (\ref{eq:MASO}).
%Adding the constant $\| \bx \|^2$ and rearranging the terms leads to the right hand side. 
%
%
\begin{figure}[t]
\begin{minipage}{0.5\linewidth}
    \centering
    (a)
    \includegraphics[width=0.4\linewidth]{Figs/PD_random_1.png}
    \hspace*{5mm}
    (b)
    \includegraphics[width=0.4\linewidth]{Figs/PD_random_2.png}
\end{minipage}
\begin{minipage}{0.48\linewidth}
    \caption{\small
    Power diagram (PD) partition of a $D=2$ dimensional space by a single DN unit for $R=3$ illustrating  Theorem~\ref{thm:unitPower Diagram}.
    (a) 
    The three hyperspheres (circles in two dimensions) are defined in terms of their centroids $[A]_{k,r,\bigcdot}$ (black dots) and radii $[{\rm rad}]_{k,r}$ allowing easy visualization of PDs.
    (b) 
    By simultaneously increasing all three radii by the same scaling factor until they intersect, we obtain the three chordales (generalization of bissectors for PDs) along which the region boundaries are aligned 
    (see Appendix~\ref{appendix:extra_geometric} for details).\normalsize}
    \label{fig:power_diagram}
\end{minipage}
\end{figure}
%
%
% of the unit input space partitioning. That is, all inputs in $\omega_r$ will be projected via the same affine transform $\Epsilon_{k,r}$ to produce the unit output.
%We can now define the centroid and radius that will define the PD of the unit:

\begin{thm}
\label{thm:unitPD}
Unit $k$ partitions its input space according to $\PD(\mathcal{X};\{([\mu]_{k,r,\bigcdot},[{\rm rad}]_{k,r}),r=1,\dots,R\})$ (recall (\ref{eq:pd_def})).
\end{thm}
The collection of inputs having the same face allocation $\omega_r=\{\bx \in \mathcal{X} : r(\bx)=r\},r=1,\dots,R$, constitutes the $r^{\text{th}}$ {\em partition cell}. 
\begin{cor}
The input space partitioning of a DN unit with $R$ regions is composed of convex polytopes.
\end{cor}
%
%
The interplay between Proposition~\ref{prop:singleunit} and Theorem~\ref{thm:unitPD} is reinforced with the following result .
\begin{prop}
The regions of the PD from Theorem~\ref{thm:unitPD} are the vertical projection on the input space $\mathcal{X}$ of the faces of the polytope $\mathcal{P}_k$ from Proposition~\ref{prop:singleunit}. (Proof in \ref{proof:1})
\label{prop:vertical_unit}
\end{prop}
%
%In the present case, the regions are determined by the hyperspheres with center $[A]_{k,r^{\star},.}$ and radius $\big[{\rm rad} \big]_{k,r} $.
%\begin{thm}
%\cite{johnson1960advanced}
%Finally, the boundary between two adjacent regions is defined as a segment of the chordale of the two hyperspheres of those regions \cite{johnson1960advanced}.
%\end{thm}
%This point is illustrated in Fig.~\ref{fig:power_diagram}.
%\richb{i don't see how it is illustrated there}
%\subsection{Special Case: Voronoi Diagram}
%


%\begin{cor}
%\label{prop:kmean}
%DN unit $k$ with bias constrained as $[B]_{k,r}=-\frac{1}{2} \big\|[A]_{k,r,\bigcdot}\big\|^2$ 
%(and hence $[{\rm rad}]_{k,r}=0$ from (\ref{eq:bias_radius}))
%partitions its input space according to a Voroni diagram with %centroids  $[A]_{k,r,\bigcdot}$, $r=1,\dots,R$.
%\end{cor}

%In this case, the chordales delimiting the partition regions become bisectors of the neighboring centroids. 

